DeepVisualInsight: Time-Travelling Visualization for Spatio-Temporal Causality of Deep Classification Training

Understanding how the predictions of deep learning models are formed during the training process is crucial to improve model performance and fix model defects, especially when we need to investigate nontrivial training strategies such as active learning, and track the root cause of unexpected training results such as performance degeneration. In this work, we propose a time-travelling visual solution DeepVisualInsight (DVI), aiming to manifest the spatio-temporal causality while training a deep learning image classifier. The spatio-temporal causality demonstrates how the gradient-descent algorithm and various training data sampling techniques can influence and reshape the layout of learnt input representation and the classification boundaries in consecutive epochs. Such causality allows us to observe and analyze the whole learning process in the visible low dimensional space. Technically, we propose four spatial and temporal properties and design our visualization solution to satisfy them. These properties preserve the most important information when inverse-)projecting input samples between the visible low-dimensional and the invisible high-dimensional space, for causal analyses. Our extensive experiments show that, comparing to baseline approaches, we achieve the best visualization performance regarding the spatial/temporal properties and visualization efficiency. Moreover, our case study shows that our visual solution can well reflect the characteristics of various training scenarios, showing good potential of DVI as a debugging tool for analyzing deep learning training processes.

==> conclusion.tex <==
\section{Conclusion}
We propose a time-travelling solution \tool to visualize how classification predictions are formed.
\tool can serve the purpose of education, anomaly diagnose, and sampling strategy comparison for model training processes.
In this work, we formally define four properties that any visualization tools should satisfy for spatio-temporal causality analyses.
We develop \tool to satisfy them, which visualizes the layout of input samples and classification boundaries.
%Our extensive experiments show that \tool outperforms state-of-the-art tools in performances regarding the spatial and temporal properties and visualization efficiency.

%Specifically, we turn four properties into a multi-objective optimization goal in our visualization model training.
%In the future work, we will further apply \tool on other
%In the future work, we will further improve the runtime efficiency and design new techniques to better satisfy the four properties.
%\ruofan{TODO: rewrite future work} 

==> data/reconstruction <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Measure-\nment","cspan":1,"rspan":3,"markup":[4,13]},{"value":"Solution","cspan":1,"rspan":3,"markup":[2,8]},{"value":"MINST","cspan":6,"rspan":1,"markup":[5,5]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]},{"value":"","cspan":-4,"rspan":1,"markup":[]},{"value":"","cspan":-5,"rspan":1,"markup":[]},{"value":"FMINST","cspan":6,"rspan":1,"markup":[5,6]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]},{"value":"","cspan":-4,"rspan":1,"markup":[]},{"value":"","cspan":-5,"rspan":1,"markup":[]},{"value":"CIFAR10","cspan":6,"rspan":1,"markup":[5,7]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]},{"value":"","cspan":-4,"rspan":1,"markup":[]},{"value":"","cspan":-5,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":-1,"markup":[]},{"value":"","cspan":1,"rspan":-1,"markup":[]},{"value":"Early","cspan":2,"rspan":1,"markup":[5,5]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"Middle","cspan":2,"rspan":1,"markup":[5,6]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"Final","cspan":2,"rspan":1,"markup":[5,5]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"Early","cspan":2,"rspan":1,"markup":[5,5]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"Middle","cspan":2,"rspan":1,"markup":[5,6]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"Final","cspan":2,"rspan":1,"markup":[5,5]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"Early","cspan":2,"rspan":1,"markup":[5,5]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"Middle","cspan":2,"rspan":1,"markup":[5,6]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"Final","cspan":2,"rspan":1,"markup":[5,5]},{"value":"","cspan":-1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":-2,"markup":[]},{"value":"","cspan":1,"rspan":-2,"markup":[]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]},{"value":"Train","cspan":1,"rspan":1,"markup":[5,5]},{"value":"Test","cspan":1,"rspan":1,"markup":[5,4]}],[{"value":"PPR","cspan":1,"rspan":2,"markup":[4,3]},{"value":"DVI","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.997","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.999","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.995","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.996","cspan":1,"rspan":1,"markup":[7,5]},{"value":"1.000","cspan":1,"rspan":1,"markup":[6,5]},{"value":"0.992","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.957","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.949","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.996","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.991","cspan":1,"rspan":1,"markup":[7,5]},{"value":"1.000","cspan":1,"rspan":1,"markup":[6,5]},{"value":"0.974","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.968","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.962","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.981","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.976","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.999","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.985","cspan":1,"rspan":1,"markup":[7,5]}],[{"value":"","cspan":1,"rspan":-1,"markup":[]},{"value":"UMAP","cspan":1,"rspan":1,"markup":[3,4]},{"value":"0.963","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.953","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.692","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.693","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.547","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.543","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.677","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.667","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.475","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.468","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.923","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.82","cspan":1,"rspan":1,"markup":[7,4]},{"value":"0.245","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.252","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.288","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.321","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.611","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.589","cspan":1,"rspan":1,"markup":[7,5]}],[{"value":"CCR","cspan":1,"rspan":2,"markup":[4,3]},{"value":"DVI","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.007","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.006","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.001","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.002","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.0003","cspan":1,"rspan":1,"markup":[7,6]},{"value":"0.000","cspan":1,"rspan":1,"markup":[6,5]},{"value":"0.007","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.008","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.0004","cspan":1,"rspan":1,"markup":[7,6]},{"value":"0.0002","cspan":1,"rspan":1,"markup":[7,6]},{"value":"0.000","cspan":1,"rspan":1,"markup":[6,5]},{"value":"0.008","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.0002","cspan":1,"rspan":1,"markup":[7,6]},{"value":"0.0022","cspan":1,"rspan":1,"markup":[7,6]},{"value":"0.004","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.003","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.0005","cspan":1,"rspan":1,"markup":[7,6]},{"value":"0.002","cspan":1,"rspan":1,"markup":[7,5]}],[{"value":"","cspan":1,"rspan":-1,"markup":[]},{"value":"UMAP","cspan":1,"rspan":1,"markup":[3,4]},{"value":"0.07","cspan":1,"rspan":1,"markup":[7,4]},{"value":"0.074","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.349","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.346","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.474","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.472","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.26","cspan":1,"rspan":1,"markup":[7,4]},{"value":"0.263","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.701","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.688","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.562","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.562","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.598","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.589","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.700","cspan":1,"rspan":1,"markup":[6,5]},{"value":"0.691","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.742","cspan":1,"rspan":1,"markup":[7,5]},{"value":"0.718","cspan":1,"rspan":1,"markup":[7,5]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"normal","fontStyle":"","textDecoration":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","backgroundColor":""}},{"style":{"fontWeight":"normal","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"normal","fontStyle":"","textDecoration":"","color":"rgb(0, 0, 0)","backgroundColor":""}},{"style":{"fontWeight":"normal","fontStyle":"","textDecoration":"","color":"rgb(0, 0, 0)"}}]},"options":{"table_caption":"","table_label":"tab:my-table"}}

==> data/temporal-nn <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal","bold":true},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"right","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"right","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"right","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"right","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"right","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"right","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"#neighbour","cspan":1,"rspan":1,"markup":[1,10]},{"value":"Solution","cspan":1,"rspan":1,"markup":[1,8]},{"value":"MINST","cspan":1,"rspan":1,"markup":[1,5]},{"value":"FMINST","cspan":1,"rspan":1,"markup":[1,6]},{"value":"CIFAR10","cspan":1,"rspan":1,"markup":[1,7]}],[{"value":"k=10","cspan":1,"rspan":3,"markup":[1,4]},{"value":"transfer learning \n+ temporal loss","cspan":1,"rspan":1,"markup":[1,34]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"-0.3967","cspan":1,"rspan":1,"markup":[1,7]}],[{"value":"","cspan":1,"rspan":-1,"markup":[]},{"value":"transfer learning","cspan":1,"rspan":1,"markup":[1,17]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"-0.34","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"","cspan":1,"rspan":-2,"markup":[]},{"value":"non-transfer learning","cspan":1,"rspan":1,"markup":[1,21]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"k=15","cspan":1,"rspan":3,"markup":[1,4]},{"value":"transfer learning \n+ temporal loss","cspan":1,"rspan":1,"markup":[1,34]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":-1,"markup":[]},{"value":"transfer learning","cspan":1,"rspan":1,"markup":[1,17]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":-2,"markup":[]},{"value":"non-transfer learning","cspan":1,"rspan":1,"markup":[1,21]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"k=15","cspan":1,"rspan":3,"markup":[1,4]},{"value":"transfer learning \n+ temporal loss","cspan":1,"rspan":1,"markup":[1,34]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":-1,"markup":[]},{"value":"transfer learning","cspan":1,"rspan":1,"markup":[1,17]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":-2,"markup":[]},{"value":"non-transfer learning","cspan":1,"rspan":1,"markup":[1,21]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},null]},"options":{"table_caption":"","table_label":"tab:my-table"}}
